FirstSwap: Pre-Consensus Trade Approvals for Decentralized Market Design

Decentralized exchanges typically give traders no execution guarantee until a block is finalized. In the meantime, external prices move, traders strategically delay submission, and block producers can influence inclusion and ordering. We introduce FirstSwap, a DEX built on a constant-function market maker pricing curve that gives traders an early pre-approval before consensus, guaranteeing inclusion and execution within their submitted price limit, with final ordering determined by limit prices rather than by a block producer. We demonstrate the benefits of trade pre-approvals in an economic model combining auction theory with CEX-DEX arbitrage. When the CEX price changes gradually, FirstSwap rewards earlier traders with better prices, discouraging strategic delay and yielding higher social welfare and gains to AMM liquidity providers than a batch auction. When the CEX price jumps abruptly, FirstSwap yields higher welfare and smaller AMM losses than fair ordering. The central challenge is delivering fast trade pre-approvals without consensus. We introduce a decentralized, scaled admissibility protocol under which each validator reserves only a fraction of the available liquidity at every price. A trader obtains approval in a single round of messages with a quorum of validators. Somewhat surprisingly, despite Byzantine validators who may approve trades arbitrarily, we show that all quorum-certified trades are jointly admissible and execute within their limits. Our protocol extends naturally to a setting where buy and sell orders can be pre-approved against each other before a block is finalized.

==> econ-glossary.tex <==
\begin{table}[t]
\centering
\caption{Glossary of main notation used in \Cref{sec:auction}.}
\label{tab:econ-glossary}
\makeatletter
\begingroup
\let\@classz\@classzold
\scriptsize
\linespread{0.95}\selectfont
\renewcommand{\arraystretch}{1.0}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\begin{tabular}{@{}p{0.26\linewidth}p{0.70\linewidth}@{}}
\toprule
\textbf{Symbol / Term} & \textbf{Definition} \\
\midrule
\multicolumn{2}{@{}l}{\textbf{The \projname exchange}} \\[2pt]
$\tx = (\amt,\limit)$
  & A trade request; $\amt$: amount of assets the trader wishes to buy;
$\limit$:  max. price per unit the trader is willing to pay. \\
$p(x),P(x), x_0$
  & Price per unit after $x$ units have been bought from the pool; with cumulative payment 
$P(x)=\int_0^x p(u)\,du, x_0$ and initial pool capacity $x_0$. \\
$S$, admissible
  & Set of trade requests
    $S=\{(\amt_i,\limit_i)\}$, admissible if $\forall\,\tx_i\in S$:
    $p(\sum_{j:\limit_j\leq\limit_i}\amt_j)\leq\limit_i$.\\
\midrule
\multicolumn{2}{@{}l}{\textbf{Economic model}} \\[2pt]
%
%
%
$\mathsf m\in\{\mathrm{FS},\mathrm{FIFO},\mathrm{batch}\}$
  & Trading mechanism: FirstSwap, fair ordering, or batch auction. \\
$p_{\mathrm{ex},t},\ p_{\mathrm{ex},0}$
  & CEX price at time $t$, and its initial value. \\
$\eps_i,\ F_\eps$
  & Trader $i$'s fixed private asset valuation,
   with a mean-zero distribution having CDF $F_\eps$. \\
$\theta_{i,t},\ r,\ \eps(r)$
  & Total valuation $\theta_{i,t}=p_{\mathrm{ex},t}+\eps_i$.
    Rank $r$ is the fraction of higher-valuation traders; $\eps(r)=F_\eps^{-1}(1-r)$. \\
$q_i(\eps_i),\ x_{\mathrm{LP}}$
  & Quantity allocated to trader $i$, inventory remaining in the pool.\\
    %
$\tau,\ p_{\mathrm{bid},\tau}$
  & Submission time, submitted limit price. \\

$\Pr_{\mathrm{fill}}(p_{\mathrm{bid}}),\Pr_{\mathsf m}(r)$
  & Execution probability of a submitted order and of a trader of rank $r$ under mechanism $m$. \\
$Vol_{\mathsf m}, \mathcal W_{\mathsf m},\ \mathcal R_{\mathsf m}$
  & Total volume:
    $\int_0^1\Pr_{\mathsf m}(r)\,dr$, social welfare and AMM gains from trade for mechanism $m$. \\

\bottomrule
\end{tabular}
\endgroup
\makeatother
\end{table}

==> glossary.tex <==
\begin{table}[t]
\centering
\caption{Glossary of main notation used in \Cref{sec:protocol}.}
\label{tab:glossary}
\makeatletter
\begingroup
\let\@classz\@classzold
\scriptsize
\linespread{0.95}\selectfont
\renewcommand{\arraystretch}{1.0}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\begin{tabular}{@{}lp{9.5cm}@{}}
\toprule
\textbf{Symbol / Term} & \textbf{Definition} \\
\midrule
\multicolumn{2}{@{}l}{\textbf{Scaled Admissibility}} \\[2pt]
$n;f;q$           & Number of validators; Byzantine threshold; quorum size \\
$\eta$        & Pre-approval fraction; $\eta := (q-f)/(n-f)$.
                Each validator pre-approves at most an $\eta$-fraction
                of available capacity at each price level. \\
$\eta${-}admissible 
              & admissible when every $\tx_i \in S$ has $\amt_i$ scaled by a factor $1/\eta$.\\
\midrule
\multicolumn{2}{@{}l}{\textbf{Pre-approvals and certificates}} \\[2pt]
$\sigma_v(\tx)$
              & Pre-approval of $\tx$ by validator $v$: a signed message
                $\langle\mathsf{APPROVE},\tx\rangle$. \\
$\pi(\tx)$    & Approval certificate for $\tx$ with
                pre-approvals from $q$ distinct validators. \\
$\mathsf{A}_v$         & Local set of trade requests pre-approved by validator $v$
                in the current epoch; $\eta$-admissible by construction. \\
$\Pi_v$       & Local set of approval certificates learned by validator
                $v$ in the current epoch. \\
\midrule
\multicolumn{2}{@{}l}{\textbf{Protocol structure}} \\[2pt]
epoch         & A fixed-duration period comprising a pre-approval phase
                followed by a consensus round to decide a final block. \\
$B_v$         & Mini-block formed by validator $v$ at epoch end:
                $B_v = (\mathsf{A}_v, \Pi_v)$. \\
$\mathcal{B}$ & Final block output by MVBA: a set of at least
                $n{-}f$ well-formed mini-blocks. \\
$\mathsf{Valid}$
              & External validity predicate for MVBA; holds when
                $\mathcal{B}$ contains well-formed mini-blocks from
                $M_{B} \geq n{-}f$ validators with consistent cross-signatures. \\
$J(w)$        & Accountability function; returns the set of validators
                implicated by evidence $w$; never implicates an honest
                validator. \\
\bottomrule
\end{tabular}
\endgroup
\makeatother
\end{table}

